Deciphering Undersegmented Ancient Scripts Using Phonetic Prior

Most undeciphered lost languages exhibit two characteristics that pose significant decipherment challenges: (1) the scripts are not fully segmented into words; (2) the closest known language is not determined. We propose a decipherment model that handles both of these challenges by building on rich linguistic constraints reflecting consistent patterns in historical sound change. We capture the natural phonological geometry by learning character embeddings based on the International Phonetic Alphabet (IPA). The resulting generative framework jointly models word segmentation and cognate alignment, informed by phonological constraints. We evaluate the model on both deciphered languages (Gothic, Ugaritic) and an undeciphered one (Iberian). The experiments show that incorporating phonetic geometry leads to clear and consistent gains. Additionally, we propose a measure for language closeness which correctly identifies related languages for Gothic and Ugaritic. For Iberian, the method does not show strong evidence supporting Basque as a related language, concurring with the favored position by the current scholarship.

==> section/outdated/experiments.tex <==
\section{Experiments}
% We test our model on two languages: Gothic and Iberian. Gothic is the main testing language given that it is well studied within the historical linguistics community.  \toadd{One sentence to describe the set of Iberian experiments.}

\subsection{Gothic}
Gothic is the earliest attested language of the Germanic family~\cite{harbert.2006}.  It is an ideal testing language to approximate an attestation situation similar to most undeciphered languages due to its limited and fragmentary data sources. Despite being a low-resource language, its phonology is well researched, providing reliable ground truths for evaluation.

\paragraph{Known languages}
We choose three languages to serve as the known language for deciphering Gothic: Proto-Germanic, Old Norse and Old English. The two latter languages are early North- and West Germanic languages attested in the second half of the first milennium AD. Proto-Germanic, however, is the reconstructed ancestor language of the Germanic languages which is assume to have been spoken in northern Europe after 500 BC \cite[][p. 241]{Ringe.2017}. They present a spectrum in terms of difficulty for decipherment. Due to the factors of difference in attestation time and degree of relatedness, Gothic is closest to Proto-Germanic as it is the earliest fully attested Germanic language. Both Old Norse and Old English are more distinct from Gothic as they belong to different sub-clades within the Germanic branch. 

\paragraph{Data}
We obtain the Gothic texts from the \texttt{Wulfila}\footnote{\url{http://www.wulfila.be/gothic/download/}} project. Texts with more than 100 characters are discarded. Cognate pairings are extracted from Wiktionary's etymological sections\footnote{\url{https://www.wiktionary.org/}}. 

Gothic stems are derived based on the documentation of \texttt{Gomorphv2} on which \texttt{Wulfila}'s annotations are based.\footnote{\url{http://www.wulfila.be/gomorph/gothic/html/}} Stemmers for the known languages are designed based on the Wikipedia documentation of their grammar and phonology\footnote{ \url{https://en.wikipedia.org/wiki/Proto-Germanic_grammar};  \url{https://en.wikipedia.org/wiki/Old_Norse_morphology}; \url{https://en.wikipedia.org/wiki/Old_English_grammar}.}. All matched stems in the known language with at least four characters form the known vocabulary $\Y$. 

For transcribing the stems into IPA symbols, we use the \texttt{CLTK} library\footnote{\url{http://cltk.org/}} for Old Norse and Old English, and a rule-based converter for Proto-Germanic based on \cite[][pp. 242-260]{Ringe.2017}. The \texttt{ipapy} library\footnote{\url{https://github.com/pettarin/ipapy}} is used to obtain their phonetic features. 

Dataset statistics are provided in Table~\ref{tab:data_stats}.
\begin{table}[h]
    \begin{tabular}{lccc}
    \multirow{2}{*}{\textbf{Lang}} & Lost     & \multicolumn{2}{c}{Known} \\
                        \cline{2-4}
                          & \#tokens & \#matches   & vocab  \\
    \toprule                        
    \textbf{Gothic}                & 40,518   & -           & -           \\
    \textbf{Proto-Germanic}        & -        & 7883       & 613 \\
    \textbf{Old Norse}             & -        & 10754        & 529 \\
    \textbf{Old English}           & -        & 11067       & 627           
    \end{tabular}
    \caption{\toadd{data stats}}
    \label{tab:data_stats}
\end{table}

In addition, the original Gothic texts are only segmented into sentences, without any tokenization. To simulate situations where an ancient text is undersegmented, we create separate datasets by randomly inserting ground truth segmentations (i.e., whitespaces) with a preset probability. Table~\ref{tab:average_lengths} shows the average lengths for different whitespace ratios.
\begin{table}[h]
    \centering
    \begin{tabular}{ccccc}
        Whitespace ratio & 0\% & 25\% & 50\% & 75\% \\
        \toprule
        Avg length & 65.7  & 16.8 & 9.6 &  6.7
    \end{tabular}
    \caption{\toadd{}}
    \label{tab:average_lengths}
\end{table}

\subsection{Iberian}
%FH
Iberian is a non-Indo-European unclassified language spoken predominantly on the pre-Roman and early Roman Iberian penninsula. It became extinct during the time of the early imperial period. Little is known for certain about this language as only parts of the phonological system, some onomastic elements and its numerical system are sufficiently understood. Iberian serves as a real test scenario for our method since it is attested in undersegmented texts and has withstood many previous attempts of full decipherment.
%Iberian is a pre-Roman language spoken primarily in Northeastern Spain. \toadd{Some basic facts for Iberian} The current scholarly understanding of this ancient language is poor and only the phonological system, some onomastic elements and its numerical system are sufficiently studied, and even those aspects are still up for debate. Iberian serves as a real test scenario for our method \toadd{why}

\paragraph{Known language}
We use Latin and Basque as the known languages to compare against Iberian. Although the current consensus is that Iberian is not genetically related to any living language, there are documents and inscriptions in Latin that have matching Iberian onomastic elements. In addition, we use Basque as a valid candidate due to its close geographic distribution and the existence of various Vasco-Iberian hypotheses.

\paragraph{Data}
We use the Iberian epigraph texts provide by Hesperia\footnote{\url{http://hesperia.ucm.es/}}. To extract the matching onomastic elements between Latin and Iberian, we take the list provided by~\citet{ramos2014nuevo} and select the elements that have both Latin and Iberian correspondences. Stemming can be performed directly based on the segmentations provided by~\cite{ramos2014nuevo}. We obtain 64 unique Latin stems in total.

For Basque, we use a Basque etymological dictionary\footnote{\note{Probably need a more formal citations.} \url{https://www.bulgari-istoria-2010.com/Rechnici/baski-rechnik.pdf}}, and extract Basque words either of unknown origins or borrowed from Latin. Stemming is performed by removing the ending vowels if preceded by consonants \toadd{based on?}. 


\subsection{Systems}
We evaluate our model using different amounts of phonological knowledge for the lost language. The \texttt{base} model assumes no knowledge while \texttt{full} model has full knowledge of the phonological system and therefore the character mappings. For the Gothic experiment, we additionally experiment with a \texttt{partial} model which assumes we know the phonetic values for the characters k, l, m, etc \toadd{@fred, say a few words about the background here.}

%\toadd{Shall we introduce a baseline, or instead do a full ablation test? For one thing, there is no well-established methodology for the problem of focus in this paper, so the quality of ``baseline'' which we improvise here just for the purpose of comparison can be arbitrary and unjustified. On the other hand, even if we devise a model for baseline, it would be more or less a simplified version of the proposed approach (eg. just do exhaustive edit-distance matching w/o any linguistic knowledge injection or generative formulation), which essentially reduces the analysis to ablation test. \newline

%Baseline is introduced when we want to compare with known or obvious methods. If nothing alike exists then such comparison is not mandatory. This being said, for the same space to be allocated for analysis, it would be more educational to include full ablation tests which pronounces the role of linguistic priors baked into the model design (in which case the most ablated model naturally serves as a baseline).}

% \subsection{Training}
% We train the model using SGD with a learning rate 0.2 for all experiments. Feature embedding size is 70, and there are 7 feature groups\toadd{make sure this is consistent}, making the vector size of each IPA symbol 490. A dropout rate of 0.5 is applied after the embedding layer. A context weight of 0.2 is used all for experiments, and a constant temperature $T=0.2$ is employed. Five different insertion penalty values are used. We refer interested readers to \toadd{Appendix, annealing, downsampling.}

\subsection{Evaluation}
We evaluate the model's performance using F1 score.  Specifically, we test the model on the subset of the training corpus which has at least one cognate or loanword pairing. A predicted span is deemed correct if and only if the predicted known stem matches the ground truth stem and the span is the prefix of the ground truth span \toadd{maybe one example in the appendix?}. 
We run the model with 10 different random seeds and five different insertion penalty values. We report the results for the best system. More details about the training process are provided in the \toadd{appendix, annealing, downsampling}



==> section/outdated/experiments_new.tex <==
\section{Experiments}
\label{sec:experiments}

\toadd{overview paragraph}

\paragraph{Systems}
We test our model using different amounts of phonological knowledge for the lost language. The \texttt{base} model assumes no knowledge while \texttt{full} model has full knowledge of the phonological system and therefore the character mappings. For the Gothic experiments, we additionally experiment with a \texttt{partial} model which assumes we know the phonetic values for the characters k, l, m, etc \toadd{@fred, say a few words about the background here.}


\subsection{Ugaritic}
We first run a variant of our \texttt{base} model on the Ugaritic dataset \toadd{cite} to directly compare with previous works that have access to the vocabulary of the lost language. 

\paragraph{Setup}
The Ugaritic dataset is used to simulate the decipherment process for Ugaritic using Hebrew as the known language. Both languages are members of the Semitic language family. Vocabularies for both languages are provided as model input, but only a subset of them are matched cognates. 

Since there is no need to perform segmentation on this dataset, we provide ground truth spans (i.e., one single span covering the entire word) for our model. This is achieved by setting $\Pr(z^*) = 1$ for the ground truth segmentation $z^*$ in~\equationref{eq:marginal_px}. We run our model with or without incorporating the phonetic geometry \note{Mention the without model in the model section}. 


\paragraph{Results} 
As Table~\ref{tab:ugaritic} shows, without the phonetic prior, our \texttt{base} model achieves 54.6\% accuracy. The effectiveness of incorporating the phonetic geometry is confirmed by the improved accuracy at 63.9\%.  We note that our \texttt{base} model performs competitively against the best reported result by \texttt{NeuroCipher}, even though our model is developed for harsher conditions with fewer assumptions.

\begin{table}[]
    \centering
    \begin{tabular}{lc}
        \textbf{Model} & \textbf{Accuracy} \\
        \toprule
        \texttt{Bayesian} &  60.4 \\
        \texttt{NeuroCipher} & 65.9 \\
        \midrule
        \texttt{base} (no phonetics) & 54.6 \\
        \texttt{base} & 63.9
    \end{tabular}
    \caption{\toadd{}}
    \label{tab:ugaritic}
\end{table}

\subsection{Gothic}
For unsegmented or undersegmented texts, we test our model by using Gothic as the lost language.

\paragraph{Background}
Gothic is the earliest attested language of the Germanic family~\cite{harbert.2006}.  It is an ideal language to approximate an attestation situation similar to most undeciphered languages due to its limited and fragmentary data sources. Despite being a low-resource language, its phonology is well researched, providing reliable ground truths for evaluation.

\paragraph{Known languages}
We choose three languages to serve as the known language for deciphering Gothic: Proto-Germanic, Old Norse and Old English. The two latter languages are early North- and West Germanic languages %attested in the second half of the first milennium AD. 
whereas Proto-Germanic is the reconstructed ancestor language of the Germanic branch.
%which is assume to have been spoken in northern Europe after 500 BC \cite[][p. 241]{Ringe.2017}. They present a spectrum in terms of difficulty for decipherment. 
Due to the difference in attestation time and \note{degree of relatedness @fred what do you mean here?}, Gothic is closest to Proto-Germanic, % as it is the earliest fully attested Germanic language. 
while Old Norse and Old English are more distinct from Gothic. % as they belong to different sub-clades within the Germanic branch. 

\paragraph{Data}
We obtain the Gothic texts from the \texttt{Wulfila}\footnote{\url{http://www.wulfila.be/gothic/download/}} project. Texts with more than 100 characters are discarded. Cognates are extracted from Wiktionary's etymological sections\footnote{\url{https://www.wiktionary.org/}}. 

Stemmers are developed based on the documentations of \texttt{Gomorphv2} for Gothic\footnote{\url{http://www.wulfila.be/gomorph/gothic/html/}}, and relevant Wikipedia entries on their grammar and phonology for the known languages\footnote{ \url{https://en.wikipedia.org/wiki/Proto-Germanic_grammar};  \url{https://en.wikipedia.org/wiki/Old_Norse_morphology}; \url{https://en.wikipedia.org/wiki/Old_English_grammar}.}. All matched stems in the known language with at least four characters form the known vocabulary $\Y$. Dataset statistics are provided in Table~\ref{tab:data_stats}.
\begin{table}[t]
    \begin{tabular}{lccc}
    \multirow{2}{*}{\textbf{Lang}} & Lost     & \multicolumn{2}{c}{Known} \\
                        \cline{2-4}
                          & \#tokens & \#matches   & vocab  \\
    \toprule                        
    {Gothic}                & 40,518   & -           & -           \\
    {Proto-Germanic}        & -        & 7883       & 613 \\
    {Old Norse}             & -        & 10754        & 529 \\
    {Old English}           & -        & 11067       & 627           
    \end{tabular}
    \caption{\toadd{data stats}}
    \label{tab:data_stats}
\end{table}


To transcribe the stems into IPA symbols, we use the \texttt{CLTK} library\footnote{\url{http://cltk.org/}} for Old Norse and Old English, and a rule-based converter for Proto-Germanic based on \cite[][pp. 242-260]{Ringe.2017}. The \texttt{ipapy} library\footnote{\url{https://github.com/pettarin/ipapy}} is used to obtain their phonetic features. 


Since the original Gothic texts are only segmented into sentences, we create separate datasets by randomly inserting ground truth segmentations (i.e., whitespaces) with a preset probability to simulate undersegmentation scenarios. Table~\ref{tab:average_lengths} shows the average lengths using different whitespace ratios.
\begin{table}[t]
    \centering
    \begin{tabular}{lrrrr}
       \textbf{Whitespace ratio} & 0\% & 25\% & 50\% & 75\%\\
        \toprule
        \textbf{Avg length} & 65.7  & 16.8 & 9.6 &6.7
    \end{tabular}
    \caption{\toadd{}}
    \label{tab:average_lengths}
\end{table}


\subsubsection{Finding matching spans}
We first test our model's ability to provide quality candidates of matching spans.

\paragraph{Evaluation}
We evaluate the model's performance using precision at K (P@K) scores. A predicted span (i.e., the stem-segmentation pair $(y, z)$) is deemed correct if and only if the stem is correct and the the segmentation is the prefix of the ground truth.
We run the model with 10 different random seeds and five different insertion penalty values and report the results for the best system. More details about the training process are provided in the \toadd{appendix, annealing, downsampling}


\begin{table*}[t]
    \centering
    \begin{tabular}{ccccc}
        \multirow{2}{*}{\textbf{Whitespace ratio}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Known language}} \\ 
        \cline{3-5}
        \cline{3-5}
        & & {Proto-Germanic} (PG) & {Old Norse} (ON) & {Old English} (OE) \\
        \toprule
        \multirow{3}{*}{0\%} & \texttt{base} & 0.714&	0.062	&0.048\\
        & \texttt{partial} &0.843&	0.429	&0.355\\
        & \texttt{full} & 0.880	& 0.595&	0.514 \\
        \midrule\midrule        
        \multirow{3}{*}{25\%} &\texttt{base} &0.687	&0.203&	0.147\\
        & \texttt{partial} &0.752&	0.447&	0.450\\
        & \texttt{full} & 0.860	&0.616&	0.504 \\
        \midrule\midrule        
        \multirow{3}{*}{50\%} &\texttt{base} & 0.718&	0.224&	0.176\\
        & \texttt{partial} & 0.713&	0.495&	0.445\\
        & \texttt{full} &0.871&	0.707&	0.511\\
        \midrule\midrule        
        \multirow{3}{*}{75\%} & \texttt{base} & 0.751&	0.302&	0.203 \\
        & \texttt{partial} & 0.737&	0.502&	0.442 \\
        & \texttt{full} & 0.866&	0.736&	0.555\\
        \midrule\midrule        
        \end{tabular}
    \caption{\toadd{gothic main results}}
    \label{tab:gothic_main_results}
\end{table*}

\paragraph{Results}
The main results of P@10 scores are summarized in Table~\ref{tab:gothic_main_results}. Across all whitespace ratio settings, we can see that in general, having more knowledge about the phonological system for the lost language significantly improves the performance ($\texttt{base} < \texttt{partial} < \texttt{full})$. Whitespace ratio also has a direct impact on model performance. The less undersegmented the texts are (i.e., higher whitespace ratio), the higher scores the model can achieve.

The choice of the known language also plays an important role. 
On the closest language pair Gothic-Proto Germanic, P@10 is at least 0.687 even without assuming any phonological knowledge about the lost language. Using Old Norse as the known language to decipher Gothic is noticeably harder, resulting in a consistent drop of performance as opposed to using Proto-Germanic. Old English as a known language is the most difficult choice for Gothic with the lowest scores among the three tested choices. This difference in model performance confirms our understanding of these Germanic languages in terms of the similarity between their phonological systems, and reaffirms that choosing a close known language is vital for decipherment. \note{optional:
We further show in detail the P@K results for the \texttt{partial} model on Old Norse (ON) with different values of K.} 
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/topk.png}
    \caption{\toadd{}}
    \label{fig:topk}
\end{figure}




% \paragraph{Insertion mechanism and language}
% \note{To our surprise, we found that for language pairs where insertion mechanisms should be needed more, the empirical results suggest otherwise.} As Table~\ref{tab:insertion_penalty} illustrates, \toadd{describe the situation}. \toadd{Offer some sort of explanation.} 

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
%     \caption{\note{table for different hyperparameter values for insertion penalty}}
%     \label{tab:insertion_penalty}
% \end{table}

% We conducted another experiment when some oracle is added to reduce the potential for overfitting. \note{As the results suggest, having a more flexible mechanism seem to have helped.}

% \paragraph{Confidence}
% We take a closer look at how the prediction  confidence affects the model performance. More specifically, we run analysis on both the inscription level and the corpus level for the scenario with whitespace ratio 0.5. 

% On the inscription level, we look at the inscriptions with at least one \ispan{s}, and report precision at K (P@K) for the most confident \ispan{s} predicted by the model. A prediction is deemed correct if it matches any ground truth span. As Figure~\ref{fig:inscription-confidence} shows, the top 10 most confident predictions give strong performance for most setups except for the hardest scenarios \texttt{ang-base-p5} and \texttt{non-base-p5}. For the remaining setups, P@10 either exceeds or is close to 50\%, with the highest at 84.6\% for \texttt{pgm-full-p5}. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figs/inscription-confidence.png}
%     \caption{\toadd{}}
%     \label{fig:inscription-confidence}
% \end{figure}


% \note{Not clear here. }On the corpus level, we sort the predictions in all inscriptions\footnote{This includes inscriptions without any \ispan{s}.} by their confidence scores, and report F1 scores based on quantiles. More specifically,  Figure~\ref{fig:corpus-confidence} shows that for most setups, we can reach peak F1 score at around 90-95\% quantile, which suggests that taking the most confident predictions can deliver the best overall performance. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figs/corpus-confidence.png}
%     \caption{\toadd{}}
%     \label{fig:corpus-confidence}
% \end{figure}

\subsubsection{Finding known languages}
\label{subsub:finding_known}
For undeciphered languages, the crucial step is to find a close and known language. To address this challenge, we need to devise a metric that corresponds well with some notion of language \textit{closeness} without access to the ground truths of matching spans. We present one metric below based on the outputs of our model.

\paragraph{Metric design}
We expect that for a closer language pair, the predictions of our model will be more confident and match more characters. To capture this intuition, we design the following metric based on \textit{prediction confidence} (i.e., probability of generating this span normalized by its length) and \textit{character coverage} (i.e., what percentage of the lost texts are matched regardless of its correctness). 
Among the top 10 predictions, we only retain the predictions with confidence above a certain threshold. Then we can calculate the value of character coverage, and plot the curve using thresholds ranging from 0.3 to 1.0. Finally, we can compute the area under the curve (AUC) as the final metric.\footnote{As an extra step, the metric is divided by 0.7 since it i s the largest possible area. However, due to the presence of inflectional endings, the actual largest possible area is dependent on the stemmer and varies from language to language. Therefore, it is more meaningful to look at the relative ranking among languages instead of the absoluate number.}. 

\paragraph{Setup} We use the dataset with 50\% whitespace ratio using the \texttt{partial} model. Besides the three Germanic languages, we add Latin, Spanish, Turkish and Hungarian as the known language. For the new additions, we use the Snowball stemmers \toadd{cite} and Epitran for IPA transcriptions \toadd{cite}. The most frequent 600 stems in the Book of Genesis \toadd{cite} with at least 4 characters form the known vocabulary. 

\paragraph{Results} As Table~\ref{tab:indicator} and Figure~\ref{fig:indicator} \toadd{increase color contrast} show, Proto-Germanic is the best choice for Gothic by a noticeable margin, followed by Old English and Old Norse. The remaining choices are significantly worse, reflecting the fact the they are either from a more distant branch (Latin and Spanish in the Romance language branch) or a different family (Turkish and Hungarian from the Turkic and the Uralic families, repsectively). These results show that at least for Gothic, this metric does correlate well with our understanding of language closeness.

\begin{table}
    \centering
    \begin{tabular}{lc}
         \textbf{Language} &  \textbf{AUC}\\
         \toprule
          PG & 0.231 \\
          ON & 0.111 \\
          OE & 0.121 \\
          Latin & 0.065 \\
          Spanish & 0.074 \\
          Turkish & 0.055 \\
          Hungarian &  0.062
    \end{tabular}
    \caption{\toadd{}}
    \label{tab:indicator}
\end{table}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/indicator.png}
    \caption{\toadd{}}
    \label{fig:indicator}
\end{figure}

\subsection{Iberian}
Lastly, we test our model on Iberian, an undersegmented and undeciphered language.
\paragraph{Background}
%FH
Iberian is a non-Indo-European unclassified language spoken predominantly on the pre-Roman and early Roman Iberian penninsula. %It went extinct during the time of the early imperial period.
Little is known for certain about this language as only the phonological system, some onomastic elements (i.e., proper names) and its numerical system are sufficiently understood. Iberian serves as a real test scenario for our method since it is attested in undersegmented texts and has withstood many previous attempts of full decipherment.
%Iberian is a pre-Roman language spoken primarily in Northeastern Spain. \toadd{Some basic facts for Iberian} The current scholarly understanding of this ancient language is poor and only the phonological system, some onomastic elements and its numerical system are sufficiently studied, and even those aspects are still up for debate. Iberian serves as a real test scenario for our method \toadd{why}

\subsubsection{Onomastic elements}
Although the current consensus is that Iberian is not genetically related to any living language, there are documents and inscriptions in Latin that have matching Iberian onomastic elements. We use these elements to first validate our model.


\paragraph{Dataset}
We use the Iberian epigraph texts provide by Hesperia\footnote{\url{http://hesperia.ucm.es/}}. To extract the matching onomastic elements between Latin and Iberian, we take the list provided by~\citet{ramos2014nuevo} and select the elements that have both Latin and Iberian correspondences. Stemming can be performed directly based on the segmentations provided by~\cite{ramos2014nuevo}. We obtain 64 unique Latin stems in total.

\paragraph{Results}
Figure~\ref{fig:xib_onomastic} shows the P@K scores for the \texttt{base} and the \texttt{full}  models. P@10 reaches 50.8\% and 67.8\% for \texttt{base} and \texttt{full} models, respectively, validating our model's ability to correct identify matching onomastic elements.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/xib_topk.png}
    \caption{\toadd{}}
    \label{fig:xib_onomastic}
\end{figure}

% \begin{table}[]
%     \centering
%     \begin{tabular}{ccc}
%          \textbf{Model} & \texttt{base} & \texttt{full} \\
%          \toprule
%          \textbf{F1} & 0.258 &  0.402
%     \end{tabular}
%     \caption{\toadd{}}
%     \label{tab:xib_onomastic}
% \end{table}

\subsubsection{?Basque and beyond?}
We proceed to follow the procedure in~\ref{subsub:finding_known} to see find any good candidates for the known language. 

For Basque, we use a Basque etymological dictionary\footnote{\note{Probably need a more formal citations.} \url{https://www.bulgari-istoria-2010.com/Rechnici/baski-rechnik.pdf}}, and extract Basque words either of unknown origins or borrowed from Latin. Stemming is performed by removing the ending vowels if preceded by consonants \toadd{based on?}. 

% \begin{table}[]
%     \centering
%     \begin{tabular}{ccc}
%         language/vocab & size & AUC \\
%         lat-ono & 64 & 0.200  \\
%         eus-pos & 266 & 0.295 \\
%         eus-neg & 485 & 0.384 \\
%         lat-gen & 600 & 0.239 \\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}


\subsection{Updates}
\paragraph{100\% whitespace ratio experiments} P@10 are reported in Table~\ref{tab:gothic_100}.
\begin{table}[]
    \centering
    \begin{tabular}{ccc}
        \textbf{Lang} & prior model & this model (base) \\
        \toprule
        Proto-Germanic &  0.753 &  0.872 \\
        Old-Norse & 0.543 &  0.534 \\
        Old-English & 0.313 & 0.363
    \end{tabular}
    \caption{Caption}
    \label{tab:gothic_100}
\end{table}
% We use Latin and Basque as the known languages to compare against Iberian.  In addition, we use Basque as a valid candidate due to its close geographic distribution and the existence of various Vasco-Iberian hypotheses.

==> section/outdated/introduction.tex <==

\section{Introduction}


% \note{My proposed writing flow goes like this:
% \begin{itemize}
%     \item[1] Introduce the phenomenon of scriptio continua, and relevantly, undersegmentation in many ancient texts or just morphologically super complicated structure.
%     \item[2] Highlight the technical challenges it brings. The combination of possible spans (the unsupervised nature), the presence of non-identifiable spans including inflectional endings that are usually not treated as evidence supporting any decipherment effort.
%     \item[3] ?? A concise account of what counts as a good decipherment: 1. bijectivity of character mapping. 2. Monotonicity. 3. locality of character mapping. 4. plausibility -- similar sounds in the lost language should be mapped to similar sounds in the known language. 5. A decent amount of coverage to demonstrate the regularity of such mappings.
%     \item[4] Introduce our proposal: a heavily phoentically/linguistically regularized CNN-based model, under a generative framework, trained to identify as many words as possible with as high confidence as possible.
%     \item[5] Summary of results and conclusions. Emphasis on Gothic as the core case study.
% \end{itemize}
% }

% %New Intro paragraph

% Traditional decipherment has thus very much relied on comparative evidence and patterns that could be detected by the human researcher. Many decipherment problems present today, however, impose challenges that are increasingly difficult for a single researcher to overcome. With the advance of computational methods, it is now possible to employ techniques that make it possible to attack the most challenging problems in decipherment left today. It needs to be stressed that traditional methods should not be abolished but integrated as a basis of a powerful computational tool which can build upon this knowledge.
% One of the obstacles present in the current unsolved decipherment problems is that many undeciphered languages do not exhibit clear word segmentations which makes the subsequent identification of words and potential congnates in other languages difficult. In the paper at hand, we present a computational model which seeks to decipher languages only attested in unsegmented texts.
















==> section/outdated/method.tex <==
\section{Method}

\subsection{Data}
\paragraph{Bible.} We downloaded the Gothic and the German Bible from the \textit{Unbound Bible} website.\footnote{\url{http://unbound.biola.edu/index.cfm?method=downloads.showDownloadMain}}
The Gothic Bible was used in the online version provided by the University of Antwerp (Belgium),\footnote{\url{http://www.wulfila.be}} based on the edition of \citet{streitberg1919gotische}. This book represents one of the major sources of knowledge about Gothic, as it includes the remains of a Bible translation made in the 4th century AD by the Visigothic bishop Wulfila (Ulfilas) as they arrived to us through later copies, written in northern Italy during the period of Ostrogothic rule (i.e. early 6th century): the \textit{Codex Argenteus}, the \textit{Codex Amborsianus}, the \textit{Codex Carolinus} and the \textit{Speyer fragments}, discovered only in 1970.
The German Bible is the online version of the Luther Bible, as it appears in the revised edition of the \textit{Lutherbibel} \citep{Lutherbibel1912}.

The two texts were aligned, normalized and tokenized through regular expressions and converted into IPA characters. The Gothic Bible was converted to IPA through regular expressions based on Gothic phonology as provided by \citet{miller.2019, braune.2004} whereas for the German convertion we utilized \textit{Epitran}.\footnote{\url{https://github.com/dmort27/epitran}} Because the downloaded version of the Gothic Bible came in Latin script, we generated a parallel Gothic script version through regular expressions.

\paragraph{Dictionary.} In order to generate the ground truth, we built a dictionary of Gothic terms with their respective German cognates. To this end, we extract from the Gothic dictionary by \citet{rajki2004gothic} all terms for which a German form is available. To increase coverage, we also scrapped Wiktionary,\footnote{\url{ https://en.wiktionary.org} accessed: 2019-12-01} which was already previously used in computational historical linguistics \citet{Hartmann.2019}.

\paragraph{Mapping.} The goal of the dictionary is to associate the Gothic terms in the Bible with the respective German forms, which need in turn to be mapped to the terms in the German Bible. To maximize the coverage, the mapping is performed on the lemmatized forms, which are obtained using lemmas extracted from Wiktionary for Gothic and using NLP-Cube\footnote{\url{https://github.com/adobe/NLP-Cube}} for German.



==> section/outdated/model.tex <==
\section{Model}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\Span}{\mathcal{S}}
\newcommand{\x}[1]{x^{#1}}
\newcommand{\xs}{\x{s}}
\newcommand{\xsi}{\x{s_i}}
\newcommand{\xsb}{\x{\bar{s}}}
\newcommand{\Xwt}{X[w_t]}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\ispan}{matched span}
\newcommand{\Ispan}{Matched span}
\newcommand{\nispan}{unmatched span}
\newcommand{\lst}[2]{[#1_1, #1_2, \dots, #1_#2]}
\newcommand{\lost}{\mathfrak{L}}
\newcommand{\known}{\mathfrak{K}}
\newcommand{\IPA}{\textit{IPA}}
\newcommand{\other}{\textbf{O}}
\newcommand{\tagend}[1]{\textbf{E}_\textbf{#1}}
\newcommand{\pnis}{p_{0}}
\newcommand{\equationref}[1]{Equation~(\ref{#1})}
\newcommand{\score}{\texttt{score}}
\newcommand{\coverage}{\texttt{coverage}}
\newcommand{\zo}{\substack{z\in Z \\ z=\other}}
\newcommand{\znoto}{\substack{z\in Z \\ z\neq\other}}
\newcommand{\E}{\mathop{}{\mathbb{E}}}
\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\cik}{c_i^{\known}}
\newcommand{\cjl}{c_j^{\lost}}
\newcommand{\nonctxp}{\Pr_{\text{nonctx}}}
\newcommand{\ctxp}{\Pr_{\text{ctx}}}
\newcommand{\nonctxpdot}{\Pr_{\text{nonctx}}(\cdot)}
\newcommand{\ctxpdot}{\Pr_{\text{ctx}}(\cdot)}

\RB{Please do not use the term "identifieable" since it has other meanings. use for instance "matched"}

% \begin{strip}

% \begin{tcolorbox}[colback=white]
% $\Pr(X) = \sum_{Z}\Big[\prod_{z\in Z} \Pr(z)\Big] \Big[\prod_{\zo}\pnis\Big] \Big[\prod_{\znoto}\Pr(x_z|z)\Big] \nonumber$
% \begin{infobox}
% Latent span sequence
% \end{infobox}

% $\Pr(x_z | z) \propto \sum_{y\in\Y} \Pr(x_z | y, z)$
% \begin{infobox}
% Latent span sequence
% \end{infobox}

% $\Pr(x | y, z) \approx \max_a \prod_\tau \Pr(x_{a_\tau} | y_\tau)$
% \begin{infobox}
% Latent span sequence
% \end{infobox}

% $\Pr(x_{a_\tau} | y_\tau)$
% \begin{infobox}
% Latent span sequence
% \end{infobox}

% $\Pr\nolimits^{(x)}(x_{a_\tau} | y_{\tau}) = \lambda_{\text{ctx}}\cdot\ctxp\nolimits^{(x)}(\cjl |y_\tau) 
%     +\ (1-\lambda_{\text{ctx}} )\cdot \nonctxp\nolimits^{(s)}(\cjl | \cik)$
% \begin{infobox}
% Latent span sequence
% \end{infobox}

% $\nonctxp(\cjl | \cik) &\propto \exp\big(\frac{E^{\lost}(\cjl) \cdot E^{\known}_{\IPA}(\cik)}{T}   \big)$
% \begin{infobox}
% Latent span sequence
% \end{infobox}

% $\ctxp(\cjl | y_\tau = \cik) &\propto \exp\big(\frac{E^{\lost}(\cjl) \cdot h_\tau( y ) }{T}  \big)$
% \begin{infobox}
% Latent span sequence
% \end{infobox}

% \end{tcolorbox}
% \end{strip}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.65\linewidth]{figs/decipherment_modeling.pdf}
    \caption{Overview of our generative modeling procedure. See text for more details.} %We start by introducing a latent sequence indicating spans in lost language that match cognates, then identify potential cognate pairs indicated by edit-distances. In modeling character mapping, we consider both contextualized and non-contextualized cases. We also employ IPA embeddings to reflect phonetic resemblance between lost and known language characters, as part of the parametrization design. See text for more details.}
    \label{fig:model_overview}
\end{figure*}


We design a neural model for the automatic identification of  cognates\footnote{Throughout this paper, the term \emph{cognate} also refers to loanwords, as both cognates and loanwords feature regular sound correspondences.} directly from unsegmented or undersegmented texts. At a high level, the model is trained under a generative framework to maximize the quality of the identified cognates while adhering to some basic principles of decipherment as detailed by \citet{luo2019neural}. The design for model paremeterization is guided by IPA representations that exploit the natural geometry existent in phonetics. 

% \consider{[YC: Overall this is a complicated modeling procedure involving multiple components and parameters as introduced throughout subsequent sections, each of which accounts for some linguistic prior. I wonder if a high-level summary of such correspondences between model components and linguistic knowledge should in place (maybe in the form of a table).]}

% \RB{I cannot agree more. It is a must to add such a figure, with appropriate explanations}

% \draft{
% Any successful decipherment effort needs to capture the following properties.
% \begin{itemize}
%     \item Bijectivity. For alphabetically writing systems, character mappings should be close to bijective.
%     \item Monotonicity.
%     \item Locality. The vast majority of sound correspondences happen locally, without long term dependencies.
%     \item Plausibility. Drastic divergence of two similar sounds is rare.
%     \item Regularity. The Neogrammarian hypothesis dictates that sound change suffers no exception.
%     %Comment FH: We should rephrase the last point a bit to make it align with more recent theories of how sound change works. I can do that.
% \end{itemize}
% We carefully design a neural model that can take into account all the properties above. \toadd{add more about the generative framework.}
% }
We organize this section as follows: the problem setting is introduced in \secref{subsec:problem_setting}; the generative framework is presented in \secref{subsec:generative}; our full training objective is detailed in \secref{subsec:objective}; model parameterization is implemented in \secref{subsec:parameterization}; and finally we describe training and inference procedures in \secref{subsec:training_inference}. 

\subsection{Problem setting}
\label{subsec:problem_setting}
We are given a list of \emph{unsegmented} or \emph{undersegmented} texts $\X = \set{X}$ in the lost language, and a vocabulary, i.e., a list of \emph{tokens} $\Y = \set{y}$ in the known language. For each lost text $X$, the goal is to identify a list of non-overlapping spans $\set{x}$ that correspond to cognates in $\Y$. We refer to these spans as \textbf{\ispan{s}}. In contrast, we refer to any remaining character as \textbf{\nispan{s}}.


% \toadd{Clarify that $y$ is actually a stem and maybe explain why a bit.}
The known vocabulary $\Y$ consists of \emph{stems} instead of \emph{full words}. The reason is that cognate pairings are typically done on the stem level without their morphological information, since morphological affixes are either subject to much diachronic change which typically are not preserved equally well as the stems, or downright incomparable because there is no genetic relationship between the two languages in question.

We denote the character sets of the lost and the known languages by $C^\lost =\set{c^{\lost}}$ and $C^\known = \set{c^{\known}}$, respectively.
To exploit the phonetic prior, IPA transcriptions are used for the known language, $C^\known$, while orthographic characters are used for the lost, $C^\lost$. 

\subsection{Generative framework}
\label{subsec:generative}
\begin{figure*}
    \centering
    \includegraphics[width=0.75\linewidth]{figs/placeholder/overview.png}
    \caption{\note{This is an overview.}}
    \label{fig:overview}
\end{figure*}

\paragraph{Overview} The overall model design procedure of our model is summarized in~\ref{fig:model_overview}. In a nutshell, we design the following generative framework for the extraction of identifiable spans.
The identifiability of any span is indicated by a sequence of latent variable $z$, and we use $x_z$ to explicitly refer to the span of text corresponding to $z$. With a sparsely-tagged sequence $Z=\set{z}$, we can demarcate the boundaries of the \ispan{s}. More specifically, we tag any \emph{single} character in a \nispan{} with $z=\other$ and the \emph{ending} character of any \ispan{} of length $l$ with $z=\tagend{l}$, where $m\leq l\leq M$ is in a preset range (see Figure~\ref{fig:overview} for a concrete example).\footnote{The tags for the non-ending characters in an \ispan{} is deterministically and therefore tacitly implied.}

Any character in the \nispan{} is assumed to be independently and identically distributed (i.i.d.) with a uniform probability $\pnis = \frac{1}{|C^\lost|}$, whereas any character sequence in the \ispan{} is generated by a latent cognate $y \in \Y$ and an alignment variable $a$. We further assume that every span is generated in an i.i.d. fashion as well. 

% This graphical model is illustrated in Figure~\ref{fig:overview}. \consider{[YC: honestly I think the current Fig 2 is a little confusing, in that x appears in both non-identifiable and identifiable boxes. Would it be more clear if we split the figure into two sub-figures? Also, it might be more instructive to show formula first, ending with something like ``our model can be summarized in Fig. 2''.]}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/placeholder/graphical.png}
%     \caption{\note{graphical model presentation}}
%     \label{fig:graphical}
% \end{figure}

Under this framework, we arrive at the following derivation for the marginal distribution:
\begin{alignat}{3}
    &&&\Pr(X)  \nonumber \\
    &=&& \sum_{Z}\Big[\prod_{z\in Z} \Pr(z)\Big] \Big[\prod_{\zo}\pnis\Big] \Big[\prod_{\znoto}\Pr(x_z|z)\Big]
    \label{eq:marginal_px}
\end{alignat}
For every possible tag sequence $Z$, we need to compute the probabilities of generating $Z$, and the characters in \nispan{s} and in \ispan{s}, respectively.

\paragraph{\Ispan{s} and edit distance} \consider{[YC: how about ``Identifiable spans imputation (or inference)''?]}
For \ispan{s} (i.e., $z=\tagend{l}$), we need to consider two latent variables: $y$ for a corresponding known cognate, and $a$ for the underlying alignment between $x$ and $y$. 

% For the known cognate $y$, we consider all potential candidates and derive the following:
% \begin{align}
%     \Pr(x_z | z) &=  \sum_{y\in\Y} \Pr(y)\cdot\Pr(x_z |y, z) \nonumber\\
%     &\propto \sum_{y\in\Y} \Pr(x_z | y, z) \label{eq:p_x_z}
% \end{align}

% Note that we additionally assume a uniform distribution for the prior $\Pr(y)$.

For the known cognate $y$, we consider all potential candidates as well their alignments $a$ with the lost language and derive the following:
\begin{align}
 \Pr(x_z | z) &=  \sum_{y\in\Y} \sum_{a\in\mathcal{A}} \Pr(y)\cdot\Pr(x_z |y, z, a) \nonumber\\
 &\propto \sum_{y\in\Y} \sum_{a\in\mathcal{A}} \Pr(x_z | y, z, a) \label{eq:p_x_z} \nonumber \\
 &\approx \sum_{y\in\Y} \max_a \Pr(x | y, z, a) \nonumber \\
 & = \sum_{y\in\Y} \max_a \prod_\tau \Pr(x_{a_\tau} | y_\tau)
\end{align}
First of all, in the formulation above we made an assumption that the prior $\Pr(y)$ is uniformly distributed. Regarding the alignment $a$, we adopt an edit distance-inspired formulation to model the mapping between $x$ and $y$, which captures the dominant mechanisms involved in cognate pairings: substitutions, deletions and insertions\consider{[YC:reference available?]}. Our alignment mechanism is inspired by Connectionist Temporal Classification (CTC) \citet{graves06ctc}. Formally for $a = \set{a_\tau}$, $a_\tau$ is the aligned position for $y_\tau$ in $x$, where $\tau$ indicates the position of character. In addition, $a_\tau$ can be $\epsilon$ which indicates that $y_\tau$ is mapped to nothing in $x$ (i.e., deletion), and $a_\tau$ can be two\footnote{Insertions of even longer character sequences are rare.} adjacent indices in $x$, signifying an additional mapped character (i.e., insertion).

Alignments are considered valid if they satisfy both of the following conditions. First, they are monotonically increasing with the exception of $\epsilon$. Second, they cover every index of $x$, which means every character in $x$ is accounted for by some character in $y$. Figure~\ref{fig:edit_distance} showcases one such example.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/placeholder/edit_distance.png}
    \caption{\note{Edit distance showcase}}
    \label{fig:edit_distance}
\end{figure}

\newcommand{\subp}{\Pr\nolimits^{\text{(s)}}}
\newcommand{\insp}{\Pr\nolimits^{\text{(i)}}}

% Given the alignment between $x$ and $y$, we can factorize the pairing $(x, y)$ into character-level mappings. We further approximate $\Pr(x | y, z)$ with the max conditional probability given a valid alignment
% \begin{align}
%     \Pr(x | y, z) 
%               &\approx \max_a \Pr(x | y, z, a) \nonumber \\
%               &= \max_a \prod_\tau \Pr(x_{a_\tau} | y_\tau) \label{eq:alignment}
% \end{align}
% \consider{[YC: consider folding $a_\tau$ into Eq.\ref{eq:p_x_z}? There should be a equation that includes both $a$ and $y$ to demonstrate the overall design.]} \RB{Totally agree}
Since inserted characters have different distributional properties, we use two separate probability distributions to capture the nuances for different operations. More specifically, we use one distribution $\subp(\cdot)$ for substitutions and deletions and add another distribution $\insp(\cdot)$ to model insertions, with $a_\tau = (a_{\tau, 1}, a_{\tau, 2})$ indicating two positions. Overall, we propose the following alignment model:
\begin{align}
    \Pr(x_{a_\tau} | y_{\tau}) &= 
    \begin{cases}
        \subp(x_{a_\tau} | y_{\tau}) & \text{(substitution)}\\
        \subp(\epsilon | y_{\tau}) & \text{(deletion)} \\
        \subp(x_{a_{\tau, 1}} | y_\tau) \nonumber \\
    \cdot\alpha \insp(x_{a_{\tau, 2}} | y_\tau)\quad & \text{(insertion)}
    \end{cases}
\end{align}
where $\alpha <= 1$ is a hyperparameter to control the use of insertions. At one extreme, $\alpha=1$ treats insertions no differently than substitutions, whereas at the other extreme, $\alpha=0$ disables the use of insertions entirely.

% \begin{alignat}{3}
%     \Pr(x_{a_\tau} | y_\tau) &=&& \subp(x_{a_{\tau, 1}} | y_\tau) \nonumber \\
%     &&&\cdot\alpha \insp(x_{a_{\tau, 2}} | y_\tau)\quad  \text{(insertion)},
% \end{alignat}

% \RB{Please combine equation (4) and (5) into a single equation. If needed, add a footnote clarifying the extension to insertion}

\paragraph{Contextualization}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/figure_devoicing.pdf}
    \caption{The PGmc term *sweblaz ('sulfur') changed to Gothic \textit{swibls}. The two changes PGmc *e > Goth \textit{i} and PGmc *-z to Goth -\textit{s} have different conditions: the first is unconditioned whereas the latter change of devoicing only occurs word-finally. Thus words such as Goth \textit{hatis} nom. sg. ('hate') show this devoicing but the plural form \textit{hatiza} nom. pl. exhibits retention of inherited /\textit{z}/ word-medially.}
    \label{fig:context}
\end{figure} 

\RB{I think it will be good to find a way to group this part with the rest of the phonetic writing}
Certain sound changes are conditioned on the context. One illustrative example of word-final devoicing for Gothic is presented in Figure~\ref{fig:context}.
To maintain the regularity of character mappings while encouraging a degree of contextualized flexibility, we further define the character mapping distribution as an interpolation\footnote{We found empirically that it worked better to interpolate in the log space, i.e., $\log\Pr(\cdot) = \lambda \log\ctxpdot + (1 - \lambda) \log\nonctxpdot$. } of a contextualized distribution and a non-contextualized distribution:
\begin{alignat}{3}
    &&&\Pr\nolimits^{(x)}(x_{a_\tau} = \cjl | y_{\tau} = \cik)\nonumber  \\
    &&=&\ \lambda_{\text{ctx}}\cdot\ctxp\nolimits^{(x)}(\cjl |y_\tau = \cik) \nonumber \\
    &&&+\ (1-\lambda_{\text{ctx}} )\cdot \nonctxp\nolimits^{(s)}(\cjl | \cik) \\
    &&&\text{for } x = s \text{ or } i. \nonumber
\end{alignat}
Since $\Pr_{\text{nonctx}}(\cdot)$ does not consider contextual cues, it will assign $\cik$ to some $\cjl$ regardless of context, creating one mapped lost character for each known character. By setting $\lambda_{\text{ctx}}$ low but nonzero, we can limit the influence of contextualization, thus biasing the model to only consider the main mapped character or something representationally similar. We additionally note that the same non-contextualized distribution $\nonctxp^{(s)}$ is used for both $x = s$ and $i$. Next, we detail our design principle for parametrization of $\Pr_{\text{nonctx}}$ and $\Pr_{\text{ctx}}$.

% Note that for the last case, $\Pr_{\theta_1,\theta_2}(x_{j-1} x_{j} | y_j)$ is parameterized by two separate neural networks
% \begin{align}
%     \Pr\nolimits_{\theta_1,\theta_2}(x_{j-1} x_{j} | y_j) &= \Pr\nolimits_{\theta_1}(x_{j-1} | y_j) \cdot \Pr\nolimits_{\theta_2}(x_{j} | y_j).
% \end{align}
% This is done so that insertions and substitutions have different distributional properties.

\subsection{Phonetics-Driven Parameterization}
\label{subsec:parameterization}
\paragraph{IPA embeddings}

\RB{This Secion should have something about Phonetics in the TItle. Ideally, we will move it closer to the Model beginning. The write-up should start with giving  intuition of what we are trying to capture.  Curently it is in paragraph 2. It should be reorganized}

In order to capture the similarity within certain sound classes, we use IPA embeddings to represent each IPA character in the known language. More specifically, any known IPA character $c^\known$ is first represented by a list of attribute-value pairs, each of which describes one concrete phonetic feature group (e.g. voicing, manner, place, etc.). Each group contains a feature embedding based on its actual value. Then, we obtain the IPA embedding for $c^\known$ by concatenating all of its relevant feature embeddings. For the example in Figure~\ref{fig:IPA}, the phone /b/ can be represented as  the concatenation of the \texttt{voiced} embedding, the \texttt{stop} embedding and the \texttt{labial} embedding.
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/placeholder/IPA.png}
    \caption{\note{IPA illustration}}
    \label{fig:IPA}
\end{figure}

This compositional structure encodes the natural geometry existent in sound classes \consider{[YC: is reference available here?]} and biases the model towards utilizing such a structure. By design, the representations for /b/ and /p/ are close as they share the same values for two out of three feature groups. This is crucial for realistic character mappings, since dissimilar sounds rarely evolve into similar ones diachronically.


We denote the entire known IPA embedding matrix by $E_{\IPA}^{\known}$, and the IPA embedding for $\cik$ by $E_{\IPA}^{\known}(\cik)$.

For the lost language, we represent each character $\cjl$ as a weighted sum of IPA embeddings on the known side. Specifically,
\begin{align}
    E^{\lost}(\cjl) = \sum_i w_{i, j} \cdot E^{\known}_{\IPA}(\cik).
\end{align}

\paragraph{Character mappings}
The two character mapping distributions (contextualized or non-contextualized) are parameterized as follows. For the non-contextualized distribution $\nonctxpdot$, we use a log-linear model based on the dot product of relevant embeddings, with temperature $T$:
\begin{align}
    \nonctxp(\cjl | \cik) &\propto \exp\big(\frac{E^{\lost}(\cjl) \cdot E^{\known}_{\IPA}(\cik)}{T}   \big)
\end{align}
For the contextualized distribution $\ctxpdot$, we use the contextualized representations on the known side:
\begin{align}
    \ctxp(\cjl | y_\tau = \cik) &\propto 
    \exp\big(\frac{E^{\lost}(\cjl) \cdot h_\tau( y ) }{T}  \big),
\end{align}
where $h_\tau(y)$ is the hidden representation at position $\tau$  obtained by running a convolutional neural network (CNN) on the known string $y$. The locality constraint built into CNNs suits our purpose perfectly since the vast majority of sound changes are local in nature. We further note that this dichotomy of parameterization is done on both $\subp(\cdot)$ and $\insp(\cdot)$.  %Note that the special symbol $\epsilon$ is only present on the lost side, which is never contextualized. 

\subsection{Objective}
\label{subsec:objective}
Given the generative framework, our training objective is designed to maximize the quality of the extracted cognates, while identifying a reasonable proportion of the text and encouraging the character mappings to be bijective.

\paragraph{Quality}
We aim to optimize the \textit{quality} of \ispan{s} under the posterior distribution $\Pr(Z|X)$, measured by a scoring function $\Phi(X, Z)$. $\Phi(X, Z)$ is computed by  aggregating the likelihoods of these \ispan{s} normalized by their lengths. More formally, we have the following objective:
\begin{align}
    Q(X) &= \E_{Z\sim \Pr(Z | X)} \Phi(X, Z)\nonumber \\
         &= \frac{1}{\Pr(X)} \E_{Z\sim\Pr(X, Z)} \Phi(X, Z) \label{eq:quality}\\
    \Phi(X, Z) &= \sum_{\znoto} \phi(x_z, z) \\
    \phi(x_z, z) &= \frac{\Pr(x_z | z)}{|x_z|}
    % \phi(x_z, z) &= \Big( \frac{\Pr(x_z | z)}{|x_z|} \Big) ^ \alpha
\end{align}
% Intuitively, $\Phi(X, Z)$ is positively correlated with the per-character likelihood of generating an \ispan{}, unaffected by the \nispan{s}. \toadd{Explain $\alpha$.}
% \consider{[YC: in terms of normalizing sequential probability, I wonder it better be geometric mean instead of arithmetic (consider the case of computing sequence-level perplexity.)]}
This term encourages the model to focus only on improving the probability of generating the \ispan{s} and not the \nispan{s}.

\paragraph{Regularity and coverage}
The regularity of sound change necessitates the identification of a non-trivial proportion of the text. More specifically, we incur a penalty if the expected coverage ratio of the identified characters under the posterior distribution falls below a given threshold $r_{\text{cov}}$:
\begin{align}
    \Omega_{\text{cov}}(\X) &= \max\Big(r_{\text{cov}}-\frac{\sum_{X\in\X} \texttt{cov}(X)}{|\X|}, 0.0\Big) \label{eq:coverage}\\
    \texttt{cov}(X) &= \E_{Z\sim\Pr(Z | X)} \Psi(X, Z) \nonumber \\
                    &= \frac{1}{\Pr(X)} \E_{Z\sim\Pr(X, Z)} \Psi(X, Z) \\
    \Psi(X, Z) &= \sum_{\znoto} \psi(x_z, z) \\
    \psi(x_z, z) &= |x_z|
\end{align}
Note that the ratio is computed on the entire corpus $\X$ instead of individual texts $X$ since the coverage ratio can vary greatly for different individual texts.

\RB{We need to explain that the threshold (Which is a hyperparamater) controls the expected overlap between two languages. This parameter enables us to apply the method even when languages share some borrowings but are not clsoely related}


% Let $p'_{i}(X)$ be the posterior of the best solution for $X\leq{i}$, and $p'_{i, t}(X)$ be the best value with $t$ as the tag for $X_i$. The best solution $(Y^*, S^*, \bar{S}^*)$ can be found via the following equations
% \begin{alignat}{2}
%     \Pr(Y^*, S^*, \bar{S}^*|X) &=&&\ p'_{n}(X) \\
%     p'_i(X) &=&& \max_t p'_{i, t}(X) \\
%     p'_{i, \other} &=&&\ \pnis \cdot p'_{i - 1} \\
%     p'_{i, \tagend{k}} &=&& \max_y \frac{\Pr(\xs, y| Z=1)}{|\Y|}\cdot p'_{i - k}, \nonumber \\
%     &&&\forall k \in [m,M]
% \end{alignat}.


\RB{You need to formulate it as skewdness rather than bijectivity, because we know it is not one-to-one}

\paragraph{Bijectivity}
We introduce two terms to enforce the bijectivity of a linguistically sound character mapping. The intuition is that any lost character should be mapped to by exactly one known character, and that character mapping distributions should be sharp. Formally these two terms are imposed on the noncontextualized distribution:
\begin{align*}
    \Omega_{\text{bij}}(C^\lost, C^\known) &= \big(\sum_{c^\known} \nonctxp(c^\lost | c^\known) - 1.0\big) ^ 2 \\
    \Omega_{\text{ent}}(C^\lost, C^\known) &= \mathcal{H}\big(\nonctxp(\cdot | c^\known)\big) + \mathcal{H}\big(\nonctxp(\cdot | c^\lost)\big)
\end{align*}
where $\mathcal{H}$ denotes entropy.

% \consider{[YC: be more specific about what each term regularizes. Also explain $\mathcal{H}$ being the entropy.]}

\paragraph{Final objective}
Putting all four terms together, we have the following final objective:
\begin{alignat}{3}
    &\mathcal{S}(\X; C^\lost, C^\known)\nonumber \\
    = &\sum_{X\in\X} Q(X)
    + \lambda_{\text{cov}}\Omega_{\text{cov}}(\X) \nonumber\\
    &+ \lambda_{\text{bij}} \Omega_{\text{bij}}(C^\lost, C^\known) + \lambda_{\text{ent}}\Omega_{\text{ent}}(C^\lost, C^\known),
\end{alignat}
where $\lambda_{\text{cov}},  \lambda_{\text{bij}}$ and $ \lambda_{\text{ent}}$ are all hyperparameters.

\subsection{Training and inference}
\label{subsec:training_inference}
Training with the final objective involves either finding the best latent variable, as in~\equationref{eq:alignment}, or computing the expectation under a distribution that involves one latent variable, as in~\equationref{eq:quality} and~\equationref{eq:coverage}.
In both cases, we resort to dynamic programming for efficient computation. A similar derivation can be achieved for inference as well. We refer interested readers to \toadd{appendix} for more detailed derivations. 



==> section/outdated/related_work.tex <==
\section{Related Work}
\paragraph{Computational decipherment}
Deciphering ancient languages via computational procedures has historically been a subject of interest. One of the most well-known example in this regard is the attempt of automatically deciphering the ``Voynich manuscript'' \cite{amancio.2013,hauer.2016}, even though it remains debatable whether the Voyninch manuscript is written in a natural language \cite{schinner2007voynich}. In these works, computational methods have been used to investigate intra-textual structures to extract information on the features of the text. Due to the mysterious nature of the task, these primarily statistical studies focus on surface textual properties such as word or \emph{n}-gram frequencies and co-occurrences. Our study, however, aims at a comparative approach between languages. In doing so, meaningful information gained from related languages enriches the decipherment ability of a model.

\paragraph{Machine learning approaches}
Machine learning and statistical methods have been heavily investigated for decipherment. EM algorithms were among the first approaches to be considered \cite{knight.1999,knight.2006}, in which an EM algorithm was proposed to estimate the conversion probability from known to cipher languages. However the main focus of these early works are on man-made ciphers like substitution. \cite{kirkpatrick13decipherment} later improved upon these models and conducted experiments with a million random starts for the EM algorithm and observed performance gains with better initialization points.  Besides the commonly used EM algorithm, \cite{nuhn2013beam,hauer2014solving,kambhatla2018decipherment} considered heuristic search procedure guided an external language model as alternative for substitution decipherment.

More recently, Bayesian approaches have been developed as a more effective decipherment framework. \cite{snyder.2010} first demonstrated the feasibility of automatic decipherment of a lost language without parallel data. In their approach, a Bayesian model was carefully designed to structurally incorporate significant linguistic constraints, including customized priors for alphabet matching, incorporation of morphological structure, etc. Following this line of research, \cite{dou.2012, dou.2013, ravi.2013} further improved Bayesian approaches for decipherment. It is important to note that for all these methods, organically integrating linguistic priors with model design is a key to reaching success.

\paragraph{Recent breakthrough}
With the rapid progress in deep learning made in the past a few years, a recent breakthrough in decipherment has been made by \citet{luo2019neural}, in which a neural sequence-to-sequence model with minimum-cost flow as a training objective is proposed. Taking advantage of the expressiveness of the neural model and an EM-like training procedure, they for the first time deciphered Linear B computationally, a syllabic language related to ancient Greek. Their approach also significantly improved the accuracy over Ugaritics. Shortly after, \citet{assael2019restoring} proposed a neural sequence model, named PYTHIA, for ancient Greek inscription restoration. Although the approach is not directly aimed for decipherment, their finding that the presence of context information is a determining factor in the accuracy of epigraphic restorations is valuable for further improving decipherment methods.


%%%%%%%%%%% Initial draft
\begin{comment}
% \note{This paragraph should not be monolithic but sectioned.}
Previous studies have already attacked the problem of decipherment of unknown languages. In the 

%%%statistical/pattern based
Some of the most prominent work in this regard are the first attempts to quantitatively decipher a text in an unknown language such as the `Voynich manuscript'. Although it is debated whether the Voyninch manuscript is written in a natural language \citet{schinner2007voynich}, it proofs to be a field of study for computational decipherment applications. Studies by \citet{hauer.2016} or \citet{amancio.2013} use computational and statistical models to analyze the text. Regarding the Voynich manuscript, such studies use computational methods to investigate intra-textual structures to extract information on the features of the text. Due to the nature of the task, these primarily statistical studies focus on textual properties such as word or n-gram frequencies and co-occurrences. Our study, however, aims at a comparative apporach between languages. By doing this, other information gained from related languages can enrich the decipherment ability of a model. 

%%%%ML
Other work has employed Bayesian inference models for decipherment \cite{dou.2012, dou.2013} which were able to apply machine translation methods to translation and decipherment tasks. \citet{ravi.2013} has presented a study to further improve such Bayesian approaches. 
Studies such as \citet{snyder.2010} have applied their computational frameworks to real-world decipherment tasks. They have shown that it is possible to use non-parametric Bayesian models to decipher the Ugaritics script by identifying Hebrew cognates of Ugaritics words based on alphabetic mappings and word translations  \cite{snyder.2010}. The Bayesian approaches use the Bayesian framework to sample from sentences or bigrams and map them to cognates or words in a target language. This is different from our approach insofar as the mapping in the present approach does not rely on Bayesian inference algorithms. However, these approaches are relevant to our work since the cross-linguistic mapping performed in these studies can be taken as a starting point for a more advanced deep learning model. There are also more general inquiries looking into the possibilities of drawing on particular linguistic properties for computational decipherment: Some of the earlier studies are \citet{knight.1999} and \citet{knight.2006}. The former study is concerned with training a model for script decipherment, whereas the latter study presents decipherment models drawing upon character code conversion and phonetic decipherment methods. 
%%DeepL
As a more recent breakthrough in decipherment, \citet{luo2019neural} proposed a neural sequence-to-sequence model with minimum-cost flow as a training objective. Taking advantage of the expressiveness of the neural model and an EM-like training procedure, they for the first time deciphered Linear B computationally, a syllabic language related to ancient Greek. Their approach also significantly improved the accuracy over Ugaritics. Shortly after, \citet{assael2019restoring} proposed a neural sequence model, named PYTHIA, for ancient Greek inscription restoration. Although the approach is not directly aimed for decipherment, their finding that the presence of context information is a determining factor in the accuracy of epigraphic restorations is valuable for further improving decipherment methods.
\end{comment}







==> section/outdated/results.tex <==
\section{Results}
% \begin{table*}[t]
%     \centering
%     \begin{tabular}{ccccc}
%         \multirow{2}{*}{\textbf{Whitespace ratio}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Known language}} \\ 
%         \cline{3-5}
%         & & \textbf{Proto-Germanic} & \textbf{Old Norse} & \textbf{Old English} \\
%         \toprule
%         \multirow{3}{*}{0\%} & \texttt{base} & 0.165 & 0.013 & 0.014\\
%         & \texttt{partial} & 0.244 & 0.081 & 0.075\\
%         & \texttt{full} & 0.359& 0.173 & 0.146 \\
%         \midrule\midrule        
%         \multirow{3}{*}{25\%} &\texttt{base} & 0.276 & 0.058& 0.042\\
%         & \texttt{partial} &0.334 &0.126 & 0.122\\
%         & \texttt{full} & 0.475& 0.265 & 0.207 \\
%         \midrule\midrule        
%         \multirow{3}{*}{50\%} &\texttt{base} & 0.437 & 0.088 & 0.047\\
%         & \texttt{partial} & 0.438& 0.169& 0.164\\
%         & \texttt{full} & 0.591& 0.346& 0.262 \\
%         \midrule\midrule        
%         \multirow{3}{*}{75\%} & \texttt{base} & 0.542 & 0.128 & 0.079 \\
%         & \texttt{partial} & 0.541 & 0.225& 0.222 \\
%         & \texttt{full} & 0.682& 0.443& 0.310 \\
%         \midrule\midrule        
%         \end{tabular}
%     \caption{\toadd{gothic main results}}
%     \label{tab:gothic_main_results}
% \end{table*}


\subsection{Ugaritic}
To make comparison with previous work that has access to a lost vocabulary, we run a variant of our \texttt{base} model on the Ugaritic dataset\toadd{cite}. This dataset consists of a Ugaritic vocabulary and a Hebrew vocabulary, and only a subset of them are matched cognates. We provide ground truth spans for our model since there is no need to perform segmentation on this dataset. As Table~\ref{tab:ugaritic} shows, if provided with no phonetic geometry, our \texttt{base} model achieves ?? accuracy, and the performance is improved to ?? if it is provided. Our \texttt{base} model performs competitive against \texttt{NeuroCipher} even though our model is not developed under the same set of assumptions, utilizing no special global properties that are only valid if a lost vocabulary is provided. 
\begin{table}[]
    \centering
    \begin{tabular}{cc}
        \textbf{Model} & \textbf{Accuracy} \\
        \texttt{Bayesian} &  60.4 \\
        \texttt{NeuroCipher} & 65.9 \\
        \texttt{base} (-no phonetics) & 54.6 \\
        \texttt{base} & 63.9
    \end{tabular}
    \caption{\toadd{}}
    \label{tab:ugaritic}
\end{table}


\begin{table*}[t]
    \centering
    \begin{tabular}{ccccc}
        \multirow{2}{*}{\textbf{Whitespace ratio}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Known language}} \\ 
        \cline{3-5}
        \cline{3-5}
        & & {Proto-Germanic} (PG) & {Old Norse} (ON) & {Old English} (OE) \\
        \toprule
        \multirow{3}{*}{0\%} & \texttt{base} & 0.714&	0.062	&0.048\\
        & \texttt{partial} &0.843&	0.429	&0.355\\
        & \texttt{full} & 0.880	& 0.595&	0.514 \\
        \midrule\midrule        
        \multirow{3}{*}{25\%} &\texttt{base} &0.687	&0.203&	0.147\\
        & \texttt{partial} &0.752&	0.447&	0.450\\
        & \texttt{full} & 0.860	&0.616&	0.504 \\
        \midrule\midrule        
        \multirow{3}{*}{50\%} &\texttt{base} & 0.718&	0.224&	0.176\\
        & \texttt{partial} & 0.713&	0.495&	0.445\\
        & \texttt{full} &0.871&	0.707&	0.511\\
        \midrule\midrule        
        \multirow{3}{*}{75\%} & \texttt{base} & 0.751&	0.302&	0.203 \\
        & \texttt{partial} & 0.737&	0.502&	0.442 \\
        & \texttt{full} & 0.866&	0.736&	0.555\\
        \midrule\midrule        
        \end{tabular}
    \caption{\toadd{gothic main results}}
    \label{tab:gothic_main_results}
\end{table*}

\subsection{Gothic}
We report the precision at 10 scores (P@10) on Gothic in Table~\ref{tab:gothic_main_results}. Across all whitespace ratio settings, we can see that in general, having more knowledge about the phonological system for the lost language significantly improves the performance ($\texttt{base} < \texttt{partial} < \texttt{full})$. Whitespace ratio also has a direct impact on model performance. The less undersegmented the texts are (i.e., higher whitespace ratio), the higher scores the model can achieve.

The choice of the known language also plays a significant role. 
On the closest language pair Gothic-Proto Germanic, P@10 is at least 0.687 even without assuming any phonological knowledge about the lost language. Using Old Norse as the known language to decipher Gothic is noticeably harder, resulting in a consistent drop of performance as opposed to using Proto-Germanic. Old English as a known language is the most difficult choice for Gothic with the lowest scores among the three tested choices. This difference in model performance confirms our understanding of these Germanic languages in terms of the similarity between their phonological systems, and reaffirms that choosing a close known language is vital for decipherment. \note{optional:
We further show in detail the P@K results for the \texttt{partial} model on Old Norse (ON) with different values of K.} 
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/topk.png}
    \caption{\toadd{}}
    \label{fig:topk}
\end{figure}




% \paragraph{Insertion mechanism and language}
% \note{To our surprise, we found that for language pairs where insertion mechanisms should be needed more, the empirical results suggest otherwise.} As Table~\ref{tab:insertion_penalty} illustrates, \toadd{describe the situation}. \toadd{Offer some sort of explanation.} 

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
%     \caption{\note{table for different hyperparameter values for insertion penalty}}
%     \label{tab:insertion_penalty}
% \end{table}

% We conducted another experiment when some oracle is added to reduce the potential for overfitting. \note{As the results suggest, having a more flexible mechanism seem to have helped.}

% \paragraph{Confidence}
% We take a closer look at how the prediction  confidence affects the model performance. More specifically, we run analysis on both the inscription level and the corpus level for the scenario with whitespace ratio 0.5. 

% On the inscription level, we look at the inscriptions with at least one \ispan{s}, and report precision at K (P@K) for the most confident \ispan{s} predicted by the model. A prediction is deemed correct if it matches any ground truth span. As Figure~\ref{fig:inscription-confidence} shows, the top 10 most confident predictions give strong performance for most setups except for the hardest scenarios \texttt{ang-base-p5} and \texttt{non-base-p5}. For the remaining setups, P@10 either exceeds or is close to 50\%, with the highest at 84.6\% for \texttt{pgm-full-p5}. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figs/inscription-confidence.png}
%     \caption{\toadd{}}
%     \label{fig:inscription-confidence}
% \end{figure}


% \note{Not clear here. }On the corpus level, we sort the predictions in all inscriptions\footnote{This includes inscriptions without any \ispan{s}.} by their confidence scores, and report F1 scores based on quantiles. More specifically,  Figure~\ref{fig:corpus-confidence} shows that for most setups, we can reach peak F1 score at around 90-95\% quantile, which suggests that taking the most confident predictions can deliver the best overall performance. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figs/corpus-confidence.png}
%     \caption{\toadd{}}
%     \label{fig:corpus-confidence}
% \end{figure}

\paragraph{Indicator for closeness}
To address the challenge of not knowing a good candidate beforehand, we need to find an indicator that corresponds well with the final performance without access to ground truth. The intuition is that ??. describe the setup and alg. Present AUC for partial p5.

\begin{table}[]
    \centering
    \begin{tabular}{cc}
         \textbf{Language} &  \textbf{Score}\\
         \toprule
          PG & 0.231 \\
          ON & 0.111 \\
          OE & 0.121 \\
          Latin & 0.065 \\
          Spanish & 0.074 \\
          Turkish & 0.055 \\
          Hungarian &  0.062
    \end{tabular}
    \caption{\toadd{}}
    \label{tab:indicator}
\end{table}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/placeholder/indicator.png}
    \caption{\toadd{}}
    \label{fig:indicator}
\end{figure}

\subsection{Iberian}
For the Iberian experiment, we first validate the model by running it against the known Iberian onomastic elements that are also recorded in Latin. As Table~\ref{tab:xib_onomastic} shows, the \texttt{full} model delivers a strong performance with F1 score at 0.402 and the \texttt{base} model gives a decent score of 0.258. 

\begin{table}[]
    \centering
    \begin{tabular}{ccc}
         \textbf{Model} & \texttt{base} & \texttt{full} \\
         \toprule
         \textbf{F1} & 0.258 &  0.402
    \end{tabular}
    \caption{\toadd{}}
    \label{tab:xib_onomastic}
\end{table}

\note{not clear here.} We then proceed to test Basque as the known language. Since we do not have the ground truth pairings, we use some Latin texts with a similar distributional property as the Iberian dataset to serve as the control group\footnote{We take the first sentences from the \textit{Book of Genesis} to match the total segment count and use a whitespace ratio of 0.75 to match the average segment length.}. The Basque vocabulary is partitioned into two subsets --- one consisting of words of Latin origin (\texttt{eus-lat}) , and the other of unknown origin (\texttt{eus-unk}) . Latin texts are partitioned into two as well --- one for texts with words Basque has borrowed (\texttt{lat-pos}) and the other without  (\texttt{lat-neg}). As Figure~\ref{fig:lat-eu} shows, among the most confident predictions, a significantly higher ratio of \texttt{eus-lat} words are found in \texttt{lat-pos} than in \texttt{lat-neg}. The Iberian dataset (\texttt{xib}) appears to have a similar curve as \texttt{lat-neg} but have a noticeably higher ratio of \texttt{eus-unk} words for the most confident predictions. \toadd{ramifications?}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/lat-eu.png}
    \caption{\toadd{}}
    \label{fig:lat-eu}
\end{figure}
\paragraph{}

\subsection{Ablation study}
\toadd{Ablation study to showcase the effectiveness of IPA embeddings.}
